Aggregation in the Mirror Space (AIMS): Fast, Accurate Distributed Machine Learning in Military Settings

Distributed machine learning (DML) can be an important capability for modern military to take advantage of data and devices distributed at multiple vantage points to adapt and learn. The existing distributed machine learning frameworks, however, cannot realize the full benefits of DML, because they are all based on the simple linear aggregation framework, but linear aggregation cannot handle the $\textit{divergence challenges}$ arising in military settings: the learning data at different devices can be heterogeneous ($\textit{i.e.}$, Non-IID data), leading to model divergence, but the ability for devices to communicate is substantially limited ($\textit{i.e.}$, weak connectivity due to sparse and dynamic communications), reducing the ability for devices to reconcile model divergence. In this paper, we introduce a novel DML framework called aggregation in the mirror space (AIMS) that allows a DML system to introduce a general mirror function to map a model into a mirror space to conduct aggregation and gradient descent. Adapting the convexity of the mirror function according to the divergence force, AIMS allows automatic optimization of DML. We conduct both rigorous analysis and extensive experimental evaluations to demonstrate the benefits of AIMS. For example, we prove that AIMS achieves a loss of $O\left((\frac{m^{r+1}}{T})^{\frac1r}\right)$ after $T$ network-wide updates, where $m$ is the number of devices and $r$ the convexity of the mirror function, with existing linear aggregation frameworks being a special case with $r=2$. Our experimental evaluations using EMANE (Extendable Mobile Ad-hoc Network Emulator) for military communications settings show similar results: AIMS can improve DML convergence rate by up to 57\% and scale well to more devices with weak connectivity, all with little additional computation overhead compared to traditional linear aggregation.

==> abstract_v1.tex <==
\begin{abstract}
%Mainly about our design as of now. Add problem specification.

Distributed machine learning (DML) can be an important capability for modern military to take advantage of data and devices distributed at multiple vantage points to adapt and learn. The existing distributed machine learning frameworks, however, cannot realize the full benefits of DML, because they are all based on the simple linear aggregation framework, but simple, linear aggregation cannot handle military-setting challenges, when learning data at different devices are heterogeneous and the ability for devices to communicate is substantially limited.

The key aspect of our design is that in aggregating steps, instead of taking a linear average of received models like all previous work, we instead take a quasi-arithmetic mean of the received values. We specifically focus on the weighted power mean (WPM). This can be viewed as a form of distributed mirror descent, where the quasi-arithmetic mean aggregation step is a linear averaging in the mirror descent dual space. %design section
Our theoretical convergence bounds recover the same big \(O\) bounds as numerous papers in both distributed machine learning and mirror descent. The bound also produces theoretical justification for the improved handling of differing local models: when a weighted power mean with power \(p\) is used under constant learning rate \(\eta\), the bound is \(O(m^{\frac{p+2}{p+1}})\), and can thus be improved by selecting larger \(p\). %theory section
Additionally, through extensive experiments on the Extendable Mobile Ad-hoc Network Emulator, we show that when \(p>1\), our design can improve the convergence speed of the model by up to 57\% and it also empirically scales well to more devices in low-communication environments%under time-varying networks
, all with little additional computation overhead compared to traditional aggregation.  %experiment section
\end{abstract}


% \textbf{Old Abstract} Distributed machine learning (DML) over time-varying networks can be an enabler for distributed battle management (DBM) of army or air force such as drone fleeting. Realizing the benefits of the DML in the defense system can perfectly monetize intelligence and strengthen the armed forces. It establishes a network for time-varying network in the army with dynamic coordination between complex processes to effectively edge out the enemies. However, this commonly used weighted arithmetic mean model poses learning challenges in high model loss, and slow convergence speed over DBM that present both opportunities and obstacles. To address this issue, in this paper, we propose a novel non-linear class of model aggregation functions to achieve efficient DML over time-varying networks in DBM. Instead of taking a linear aggregation of neighboring models as most existing studies do, our mechanism
%     uses a nonlinear aggregation,%removed p is odd
%     a weighted power-$p$  mean (WPM) where $p$ is a positive integer, as the aggregation function of local models from neighbors. The subsequent optimizing steps are taken using mirror descent defined by a Bregman divergence that maintains convergence to optimality. In this paper, we analyze properties of the WPM and rigorously prove convergence properties of our aggregation mechanism. Additionally, through extensive experiments on the Extendable Mobile Ad-hoc Network Emulator, we show that when $p>1$, our design significantly improves the convergence speed of the model and the scalability of DML under time-varying networks compared with arithmetic mean aggregation functions, with  little additional computation overhead. 
% \end{abstract}

==> background_save.tex <==
\section{Problem Formulation and Motivation}
\label{sec:backgroud}
\subsection{Problem Formulation}
We consider distributed machine learning with $m$ devices and no central servers. In each time interval, we assume that communication channels exist between certain pairs of local devices at any time, and that the channels are symmetric. These situations are common in practical applications (\eg, autonomous reconnaissance by a UAV swarm).

Each device $i$ has its own dataset $D_i$, from which it constructs its local loss function $f_i$. Then, if the model parameters are represented by a vector $\textbf{w}\in \RR^d$, the devices aim to collaboratively solve the following unconstrained optimization problem
\begin{equation}
\label{eq:problem}
    \min F(\textbf{w}) = \sum_{i=1}^m f_i(\textbf{w}),
\end{equation}
without sharing local data.

\subsection{Motivation}
Distributed machine learning aims to solve the aforementioned problem. All three major paradigms --- parameter server, all-reduce, and decentralized --- work by calculating local gradient information and using it to update a global model (the global model is implicit in decentralized methods). When the datasets $D_i$ are Non-IID (heterogeneous) and the communication network between local devices is sparse and dynamic, local models may diverge away from each other. This is undesirable because the local gradients will longer be a good approximation to the gradient at the global model. 
% For example, consider the following toy example. 
% There are $m$ nodes each with a local value $x_i$. At each iteration, some pairs can communicate and update their local $x$ values. Find a simple function $A:\mathbb{R}^m \to \RR$ (that depends on all inputs) and algorithm that has all nodes converge to $A(x_1,x_2,...x_M)$.

% This was in fact the motivating example. Having $A(x_1,\ldots, x_M) = \frac1m \sum_{i=1}^m x_i$ would recover \du{\sout{the normal}} the normal objective in DML: finding the average of all of the local gradients and/or models. However, trying to find the average by for example taking the average of neighbor values is quite slow. We noted that letting $A= \max_{i} |x_i|$ \du{$\max |x_i|$?}was far quicker. At each iteration, for every device $i$, the new value is $x_{i,t+1} = \max_{j\in N_i(t)} |x_j|$. 

% This was obviously infeasible, while there would be very little drift, it would depend on the behavior of the largest \du{maximum?} value.
The \sys{} framework is designed to handle this scenario. The general idea of \sys{} is mapping model values to a mirror space, averaging there, and then mapping back. In this paper, we focus on using \sys{} to generalize distribution methods, which have aggregation steps of the form $x_{i,t+1} = \sum_{j=1}^m P(t)_{i,j} x_{j,t}$ where $P(t)$ is a doubly stochastic matrix representing connectivity at time $t$. Then, for example, if the mapping is $x^p$, the \sys{} framework would give a ``weighted power mean":
\begin{equation}
\label{eq:WPM}
    x_{i,t+1} = \left(\sum_{j=1}^m P(t)_{i,j} x_{j,t}^p\right)^{\frac1p}.
\end{equation}
Such mappings help reduce variance compared to traditional linear averaging. 
To build intuition, consider an example setting where device $1$ has model $w_{1,t}=3$, and device $2$ has model $w_{2,t}=11$. Assume connectivity matrix is $P(t)=\begin{bmatrix} 0.6 & 0.4\\ 0.4 & 0.6 \end{bmatrix}$, under traditional linear aggregation, this gives a final difference of $ (0.4\cdot 3 + 0.6\cdot 11) - (0.6\cdot 3 + 0.4\cdot 11) = 7.8-6.2 = 1.6$, 
while using a weighted power mean of degree $p=5$ gives a difference of $(0.4\cdot 3^5+0.6\cdot 11^5)^{\frac15}-(0.6\cdot 3^5+0.4\cdot 11^5)^{\frac15}\approx 9.93-9.16 = 0.77$. In this case, changing the value of $p$ has more than halved the final difference.

However, the weighted power mean is just a subcase of the more general strategy of averaging in a mirror descent dual space. Single-node mirror descent works with the update function $\nabla \phi(x_{t+1}) = \nabla \phi(x_t) - \eta g_t$, causing gradient steps to be taken in the dual space (the $\nabla \phi(\cdot)$ space). In the \sys{} framework, we not only take gradient in the mirror space, but also average in the mirror space. Thus, the \sys{} version of a distributed aggregation step is the following implicit equation:
\begin{equation}
    \nabla \phi(x_{i,t+1}) = \sum_{j=1}^m P(t)_{i,j} \nabla \phi(x_{j,t})
\end{equation}
Setting $\phi = \frac1{p+1}\lVert x\rVert^{p+1}$ recovers the weighted power mean in Equation \ref{eq:WPM}. The choice of $\phi$ best suited for any problem may vary, but they all converge under a uniform convexity assumption with degree $r$ at a rate of $O(\frac{1}{\sqrt[r]{T}})$ dependence as seen in Table \ref{tab:convrate}. Note that for a weighted power mean like in Equation \ref{eq:WPM}, $\phi(x) = \frac1{p+1} \lVert x\rVert^{p+1}$ has uniform convexity of degree $r=p+1$.
% Now, in order to have good convergence properties, the gradient steps should be taken in the dual ($\nabla \phi(x)$ values) space. 
% This is one drawback of previous ``distributed mirror descent" work; their averaging still happens in the primal space directly on the models~\cite{li2016,shahrampour2016, doan2018,yuan2020distributed}. 
% Because of this, the optimality condition of $\sum_{i=1}^m \nabla f_i(x)=0$ is not a stable point for typical distributed mirror descent because $\sum_{i=1}^m \nabla f_i(x)=0$ does not imply that the sum of the mirror descent steps is 0.
